Optimal Integrated Task and Path Planning and Its Application to Multi-Robot Pickup and Delivery

We propose a generic multi-robot planning mechanism that combines an optimal task planner and an optimal path planner to provide a scalable solution for complex multi-robot planning problems. The Integrated planner, through the interaction of the task planner and the path planner, produces optimal collision-free trajectories for the robots. We illustrate our general algorithm on an object pick-and-drop planning problem in a warehouse scenario where a group of robots is entrusted with moving objects from one location to another in the workspace. We solve the task planning problem by reducing it into an SMT-solving problem and employing the highly advanced SMT solver Z3 to solve it. To generate collision-free movement of the robots, we extend the state-of-the-art algorithm Conflict Based Search with Precedence Constraints with several domain-specific constraints. We evaluate our integrated task and path planner extensively on various instances of the object pick-and-drop planning problem and compare its performance with a state-of-the-art multi-robot classical planner. Experimental results demonstrate that our planning mechanism can deal with complex planning problems and outperforms a state-of-the-art classical planner both in terms of computation time and the quality of the generated plan.

==> motionplanning.tex <==
% \section{Motion Planning} 
% \label{sec-motionplanning}

% \is{AMAN: Update this section with CBS based algorithm.}

% \begin{algorithm}[t]
% \caption{Updated Multi Label $A^*$}
% \label{alg:Algorithm3}
% \begin{algorithmic}[1]
% \Procedure {Multi-Label A*}{$\mathcal{W}$, $\mathcal{L}_i$, $\mathcal{D}_i$, $\mathcal{C}$}
% \State Create a node $n_0$ with $g$ = 0, $cgi$ = 0, 
% \Statex \hspace{10pt} $f$ = $\sum_{j=0}^{j<|\mathcal{L}_i|-1}$ H($\mathcal{L}_{i,j}$, $\mathcal{L}_{i,j+1}$)
% \State Add state $p_0$ to Priority Queue Q with key as $f$.
% \While{ Q not empty}
% \State $p$ $\gets$ Q.pop()
% \If{Final Goal Reached}
% \State $\mathtt{return}$ path
% \ElsIf{Current Goal Reached}
% \State $p.cgi$ $\gets$ $p.cgi + 1$
% \Else 
% \For{ $n \in Valid\_Neighbor(p)$}
% \State Create node $p^{'}$ with $g$ = $p.g$ + $1$, $cgi$ = 
%  $p.cgi$,  $f$ = $p.g$ + H($n$, $\mathcal{L}_{i, cgi}$) + 
%   $\sum_{j=cgi}^{j<|\mathcal{L}_i|-1}$ H($\mathcal{L}_{i,j}$, $\mathcal{L}_{i,j+1}$)

% \If{ $p^{'}$ satisfies $\mathcal{C}$ and $p^{'}.g$ + H($n$, $\mathcal{L}_{i, cgi}$) $\leq$ $\mathcal{D}_{i, cgi}$ }
% \State Add node $p^{'}$ to priority queue Q.
% \EndIf
% \EndFor

% \EndIf
% \EndWhile
% \State $\mathtt{return}$ False
% \EndProcedure
% \Statex
% \end{algorithmic}
% \end{algorithm}

% \ryn{
% As a motion planner, we use an extended version of the state-of-the-art Conflict-Based Search (CBS). The vanilla CBS algorithm is a multi-agent path-finding MAPF algorithm which takes a single source and a single goal location for each robot. We extend the CBS algorithm to handle the sequence of locations for each robot. The CBS is a two-level planner where the low-level planner produces a path for individual robots, whereas the high-level planner searches a constraint tree to get the best collision-free path. We modified the low-level planner with an updated version of multi-label A*. In multi-label A*, we provide the algorithm with a workspace $\mathcal{W}$ and a sequence of locations $\mathcal{L}_i$ and deadlines $\mathcal{D}_i$ to be visited by the robot $r_i$. We also update the algorithm to handle task deadlines differently with respect to the original algorithm. We avoid an explored node in multi-label A* if its f (cost) exceeds the deadline.}

% \ryn{
% In Algorithm $\ref{alg:Algorithm3}$, $\mathcal{L}_i$ and $\mathcal{D}_i$ are the sequences of locations and their deadlines as a Queue. The Multi-label A* works similarly to original A* except when a state node reaches its current assigned destination; it checks if the currently assigned destination is an intermediate location or the final location in the $\mathcal{L}_i$. If the state node reaches the final location in the $\mathcal{L}_i$, it returns the constructed path using the current state. If the state node reaches an intermediate location in the $\mathcal{L}_i$, it changes its current assigned destination to the following location in the $\mathcal{L}_i$ queue. We use a variable $cgi$ (current goal index) to track the next location to visit. The f(n) cost also gets updated to handle multiple locations. We use the following heuristic function in this Algorithm}

% \ryn{
% \begin{subequations}
% \begin{align}
%         f(n) =  g(n) +  H(n, \mathcal{L}_{i, cgi})  + \sum_{j=cgi}^{j<|\mathcal{L}_i|-1} H(\mathcal{L}_{i,j}, \mathcal{L}_{i,j+1}) \nonumber
% \end{align}
% \label{eq:fcost}
% \end{subequations}
% }
% \ryn{
% In the above equation, $g(n)$ denotes the distance from the source to the current location via the visited intermediate locations. $H(n, \mathcal{L}_{i, cgi})$ denotes the heuristic distance between the current node to the next goal location. The remaining term denotes the sum of heuristic costs between the next consecutive locations.}

% \ryn{
% The higher level of the Multi Label Conflict Based Search starts with an empty constraint set and uses the low level planner to compute solution for individual robots. At each iteration, it pops out lowest cost constraint set, check for conflicts, add the constraint to constraint set of conflicting agent then recomputes using low level planner. The high level planner remains the same as the original Conflict Based Search algorithm.
% }

% \ryn{
% In the following theorems, we will prove that the Multi Label Conflict Based Search produces an optimal collision free paths.}


% % \begin{theorem}
% % \label{th:th3}
% % \ryn{The updated Multi Label A* is optimal.}
% % \end{theorem}
% % \begin{proof}
% %     \ryn{
% %     Assuming, the heuristics is set 0 for the algorithm i.e. f(n) = g(n). The algorithm becomes similar to uninformed uniform cost search. It will explore the state space in best first manner and will discard the states based on constraints, hence will return a valid optimal solution.
% %     Now, if we prove that the heuristic function always underestimates the actual cost, then the multi-label A* become optimal.
% %     Let $L_i$ be the sequence of locations to visit by robot $i$ and $h(n)$ be the heuristic cost and $h^{'}(n)$ be the actual cost from a arbitrary expanded node $n$ which is going toward $L_{i, cgi}$.} Then
% %     \[  h(n) = H(n, \mathcal{L}_{i, cgi}) + \sum_{j=cgi}^{j<|\mathcal{L}_i|-1} H(\mathcal{L}_{i,j}, \mathcal{L}_{i,j+1}),
% %     \] 
% %     \[  h^{'}(n) = H^{'}(n, \mathcal{L}_{i, cgi}) + \sum_{j=cgi}^{j<|\mathcal{L}_i|-1} H^{'}(\mathcal{L}_{i,j}, \mathcal{L}_{i,j+1}) 
% %     \]
% %     \ryn{
% %     Now, in our algorithm we have used Manhattan distance as the heuristic function, therefore it is shortest possible distance between two nodes as it does not account the obstacles and the space time constraints.
% %     Therefore, }
% %     \[    H(n, \mathcal{L}_{i, cgi}) \leq  H^{'}(n, \mathcal{L}_{i, cgi}) \]
% %     \[  H(\mathcal{L}_{i,j}, \mathcal{L}_{i,j+1}) \leq H^{'}(\mathcal{L}_{i,j}, \mathcal{L}_{i,j+1}) \hfill \forall j \in [0, |\mathcal{L}| - 1) \]
% %     \ryn{Combining above two equation, we can say $h(n) \leq h^{'}(n)$ always. Therefore, multi label A* is always guaranteed to find an optimal solution.}
    
% %      \ryn{We can also prove that discarding nodes with respect to $f(n)$ instead of $g(n)$ is feasible and more efficient. Let the next location to visit and its corresponding deadline be $\mathcal{L}_{i,j}$ and $\mathcal{D}_{i,j}$ respectively. Let a node $n$ be expanded whose estimated cost fails deadline i.e. $f(n) > \mathcal{D}_{i, j}$. Since, the actual cost to reach $\mathcal{L}_{i,j}$ will always be greater or equal to estimated cost i.e.  $f^{'}(n) \leq f(n)$. Using above information, we can say $f^{'}(n) > \mathcal{D}_{i, j}$. Therefore we can safely discard node $n$. Expanding a state which has already failed the next deadline is unnecessary as all subsequent expanded state will result in failed deadline. Therefore, discarding node with respect to $f(n)$ is more efficient.
% %     }
% % \end{proof}
% % \begin{theorem}
% \label{th:th4}
% \ryn{Multi Label Conflict Based Search (ml-CBS) return an optimal solution}
% \end{theorem}
% \begin{proof}
% \ryn{
% Since the low level planner is optimal, we can substitute this information in Definition 2 and Lemma 1, and can formally prove that Multi Label CBS returns an optimal solution for both the optimization criteria.
% In simple words, Multi Label CBS explores the constraints sets tree in best first order, so the constraint sets resulting in minimal cost or minimal makespan consistent(collision free) solution from low level planner will be explored before other valid solutions. }
% \end{proof}


% \begin{comment}
%  \delete{ As a motion planner, we use an extended version of the state-of-the-art multi-robot motion planner $\textsf{M*}$~\cite{WagnerC11}.
% The M* algorithm takes as input a single goal location for each robot. 
% %We use an extended version of M*~\cite{WagnerC11} for multiple goals as motion planner. M* algorithm does multi-robot path planning efficiently for single goals. 
% For our application, we need a motion planner that can deal with multiple goals for each robot as a single robot may require to visit multiple locations in a given sequence. 
% We extend $\textsf{M*}$ to deal with a sequence of goal locations for each robot. 
% Algorithm $\ref{alg:Algorithm3}$ shows the extended version of $\textsf{M*}$ for multiple goals.
% The input to the motion planner are the workspace and sequence of locations to be visited by each robot.}

% \delete{
% In Algorithm $\ref{alg:Algorithm3}$, $\mathcal{L}_i$, the sequence of locations that needs to be visited by $r_i$, is implemented as a Queue data structure. In the algorithm, we use two sets of robots $completed$ and $working$. At any given point of execution, the set $completed$ contains all the robots for which the mission has been completed. On the other hand, the set $working$ contains those robots for which the motion plan computation has still not been completed. Initially, All the robots that do not need to visit any location are directly moved to the $completed$ set and all other robots are moved to $working$ set.}

% \delete{
% For all the working robots $r_i$, we set the first location from their queue $\mathcal{L}_i$ as their current goal locations (line 14-16). For all the robots in the set $completed$, we set their initial locations as goal locations. Now we invoke the $\mathsf{M*}$ algorithm for these goal locations and generate the collision-free trajectories in $plan$ (line 17). In this plan, different robots will reach their respective goal locations in different number of steps. From $plan$, we find the minimum index at which a working robot reaches its goal location (line 18). We call this index $mgri$. Now, for all the robots in $working$, we check if robot $r_i$ has reached its goal location at $mgri$ step. If a robot $r_i$ has reached its goal at $mgri$ step then we remove the first entry from its queue $\mathcal{L}_i$ as it has reached that location (line 21). If $\mathcal{L}_i$ has become empty, we move $r_i$ from $working$ to $completed$ (line 22-24). For the next iteration, we take all the working robot's location at $mgri$ as their initial locations (line 29) and the first location in their queue as their next goal locations (line 14-16).
% The current plan till index $mgri$ is added to the total plan for each robot (line 30). In the next iteration, we  generate the plans from this state.}

% \delete{
% Additionally,  a waiting state for the robots can be added to this planner to deal with the action primitives. It can be used in cases where at some location a robot needs to spend more time to perform an action. In our warehouse example such situations arise when a robot has reached the location it needs to pickup the object from but the object is not at that location yet.}
% \end{comment}

